MSCEqF: A Multi State Constraint Equivariant Filter for Vision-aided Inertial Navigation

This letter re-visits the problem of visual-inertial navigation system (VINS) and presents a novel filter design we dub the multi state constraint equivariant filter (MSCEqF, in analogy to the well known MSCKF). We define a symmetry group and corresponding group action that allow specifically the design of an equivariant filter for the problem of visual-inertial odometry (VIO) including IMU bias, and camera intrinsic and extrinsic calibration states. In contrast to state-of-the-art invariant extended Kalman filter (IEKF) approaches that simply tack IMU bias and other states onto the $\mathbf{SE}_2(3)$ group, our filter builds upon a symmetry that properly includes all the states in the group structure. Thus, we achieve improved behavior, particularly when linearization points largely deviate from the truth (i.e., on transients upon state disturbances). Our approach is inherently consistent even during convergence phases from significant errors without the need for error uncertainty adaptation, observability constraint, or other consistency enforcing techniques. This leads to greatly improved estimator behavior for significant error and unexpected state changes during, e.g., long-duration missions. We evaluate our approach with a multitude of different experiments using three different prominent real-world datasets.

==> preamble/preamble_compatible.tex <==

% Colour.  Used mostly for todos/notes/audits.
\usepackage{xcolor}  % Needed for colours - load before mdframed

%% RM Commenting process
%===================================================
%% comment environments {audit}
% audit.  Its an environment used for large chunks of text
\newenvironment{audit}{\color{orange}}{\color{black}}
% todo - use for a reminder of things to do.
\newcommand{\todo}[1]{{\color{red} #1}}
%% aside - a short comment to the authors, but not requiring work.
\newcommand{\aside}[1]{{\color{blue} #1}}
%% \margin{...} % a very short comment put in the margin.
\newcommand{\margin}[1]{\marginpar{\tiny #1}}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Uncomment to switch off notes
%\renewcommand{\margin}[1]{} %% Get rid of all margin comments
%\renewcommand{\todo}[1]{}%%  Get rid of todo comments
%\renewenvironment{audit}{}{} %% leave the audit text but without the colour.
%\renewcommand{\aside}[1]{} %% Get rid of all comments
%===================================================

% math symbols 
\usepackage{amssymb}
% We did use MnSymbol but this had problems with type 3 fonts.

\usepackage{amsmath}
\usepackage{mathdots}

%  this is used for \mathclap and symbol generation needed for \obb symbol.
\usepackage{mathtools} 

% for \mathbb
%\usepackage{bbm}
%\let\mathbb\mathbbm

% left indices
\usepackage{tensor}

% for \mathcal lower case
\usepackage{urwchancal}
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% allow the use of scalable vector graphics
\usepackage{graphicx}
\usepackage{ifpdf}
\ifpdf
\usepackage{epstopdf}
\epstopdfsetup{update,prepend}
\PrependGraphicsExtensions{.svg}
\DeclareGraphicsRule{.svg}{pdf}{.pdf}{% <- do not remove!
  `inkscape -z -D #1 --export-pdf=\noexpand\OutputFile
}
\fi
%% To switch off figures -
%\usepackage[demo]{graphicx} % use this to switch off figures


% theorem environments
%\usepackage{amsthm}
% -- or
%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

% list environments
\newenvironment{List}
{\begin{list}
 {[\arabic{enumi}]}
 {\usecounter{enumi}
  \settowidth{\labelwidth}{[99]}}
  \setlength{\labelsep}{1em}}
{\end{list}}


==> sections/acknowledgement.tex <==
\section*{Acknowledgement}
